COOKIEGRAPH: Understanding and Detecting First-Party Tracking Cookies

As third-party cookie blocking is becoming the norm in browsers, advertisers and trackers have started to use first-party cookies for tracking. We conduct a differential measurement study on 10K websites with third-party cookies allowed and blocked. This study reveals that first-party cookies are used to store and exfiltrate identifiers to known trackers even when third-party cookies are blocked. As opposed to third-party cookie blocking, outright first-party cookie blocking is not practical because it would result in major functionality breakage. We propose CookieGraph, a machine learning-based approach that can accurately and robustly detect first-party tracking cookies. CookieGraph detects first-party tracking cookies with 90.20% accuracy, outperforming the state-of-the-art CookieBlock approach by 17.75%. We show that CookieGraph is fully robust against cookie name manipulation while CookieBlock's acuracy drops by 15.68%. While blocking all first-party cookies results in major breakage on 32% of the sites with SSO logins, and CookieBlock reduces it to 10%, we show that CookieGraph does not cause any major breakage on these sites. Our deployment of CookieGraph shows that first-party tracking cookies are used on 93.43% of the 10K websites. We also find that first-party tracking cookies are set by fingerprinting scripts. The most prevalent first-party tracking cookies are set by major advertising entities such as Google, Facebook, and TikTok.

==> MacrosMarkup.tex <==
% For TeXshop: make it LaTeX the root file if you cmt-T here.
% !TEX root = main.tex

%%% Macros for "in progress" artefacts: colours, funny footnotes, funny endnotes, showing labels etc.
%%% MacrosMarkup Carroll Morgan 21 September 2018 and Kostas Chatzikokolakis.
\providecommand{\UsePackageFor}[2]{ \ifx#2\undefined\usepackage{#1}\fi }

\UsePackageFor{amssymb}{\boxtimes}
\usepackage[normalem]{ulem}		% For strikethroughs.
\usepackage{bbding}				% For the small pencil.
%\usepackage{dingbat}			% For pointing hand.
\usepackage{endnotes}			% For endnotes.
\usepackage{hyperref}			% For hyperlinks to and from endnotes.
\usepackage{hyperendnotes}	% Make \ref's to endnotes work correctly with hyperref.
\usepackage{pdfcolfoot}			% Fixes issues with coloured footnotes that break across pages.

% pdfcolfoot tries to restore footnote colours that break across pages, which might cause
% a colour to escape to the next footnote. So we use our own wrapper of \footnote,\footnotetext
% and enclose the footnote in a dummy FootnoteContent environment, so that the colour is restored.
% (Note: MacrosLabels applies the exact same patch for a different purpose.)
%
\ifdefined\OrigFootnote\relax\else% might be already applied by MacrosLabels
	\newenvironment{FootnoteContent}{}{}
	\let\OrigFootnote\footnote
	\let\OrigFootnoteText\footnotetext
	\renewcommand{\footnotetext}[1]{\OrigFootnoteText{\begin{FootnoteContent}#1\end{FootnoteContent}}}
	\renewcommand{\footnote    }[1]{\OrigFootnote    {\begin{FootnoteContent}#1\end{FootnoteContent}}}
\fi

%%% Colours and markups
%
\definecolor{PurplePlum}{rgb}{0.1,0,0.55} 
\definecolor{Brown}{rgb}{0.5,.25,0}
\definecolor{Orange}{rgb}{1,.3,0}
\definecolor{Gray}{rgb}{.7,.7,.7}
\definecolor{DarkGreen}{rgb}{.1,.41,.1}
%\definecolor{Black}{rgb}{0,0,0}
%\definecolor{PineGreen}{rgb}{0,0.5,0.5}
%\definecolor{Green}{rgb}{0,.5,0}

\newif\ifBleck
\newcommand\Bleck {\Blecktrue} % Carry out all deletes and replacements; remove all footnotes/endnotes; make everything black.

% To check that all colouring-calls to markup functions have been removed, disable \Bleck and enable Colour->\undef.
\newcommand\Colour[1] {\color{#1}}
%\renewcommand\Colour[1] {\undef} % Enable this to check that no colours are used by Markups.

\newcommand\PrintToCLinks{	% This prints the actual links.
  {\Colour{blue}\mbox{
    \hyperlink{w1619}{\sf$\rightarrow$~top}\quad
    \hyperlink{w1031}{\sf$\rightarrow$~toc}\quad
    \hyperlink{w1148}{\sf$\rightarrow$~lof}\quad
    \hyperlink{GreenRoom}{\sf$\rightarrow$~gr}\quad
    \hyperlink{EndNotes}{\sf$\rightarrow$~en}\quad
    \hyperlink{Sargasso}{\sf$\rightarrow$~sg}\quad
    \hyperlink{Index}{\sf$\rightarrow$~idx}
  }}
}
% http://tex.stackexchange.com/questions/201348/why-doesnt-makeatletter-work-inside-newcommand
\makeatletter % must be outside \newcommand
\newcommand\ToCLinks{
  % create "top" target
  \ifx\@onlypreamble\@notprerr		% If in document...
    \hypertarget{w1619}{}			% ...do it now.
  \else
    \AtBeginDocument{\hypertarget{w1619}{}}	% But in the preamble, delay.
  \fi

  \ifBleck\else	% 1031: Put hyperlink to ToC  and GR at bottom of every page.
    			% KOMA has \cofoot and \cefoot commands for adding a centered footer that
    			% co-exists with the page's normal footer. If available we use them.
    \ifdefined\cofoot
      \cofoot{\PrintToCLinks}
      \cefoot{\PrintToCLinks}
    \else
      \def\@oddfoot{\PrintToCLinks}
      \def\@evenfoot{\PrintToCLinks}
    \fi
 \fi
}
\makeatother

\newif\ifEndNotes % 0831: Workaround for endnotes-bug: missing ".ent" file when there are no endnotes.

\newcommand\FnSym{{\scriptsize\PencilLeftDown\kern.1em}}		% Needs bbding.
\newcommand\EnSym {{$\bigtriangledown$}}
\newcommand\Fn[1] {[\FnSym\ref{#1}]}						% For referring to footnotes.
\newcommand\En[1] {[\EnSym\ref{#1}]}						% For referring to EndNotes.
\newcommand\ENSection[1] {\par\noindent\textbf{\large #1}\par\medskip}
\newcommand\ENSubsection[1] {\par\noindent\textbf{#1}\par\medskip}
\newcommand\ENItem[1] {\item[\textbf{#1}]~\par}
%\newcommand\NA[1] {{\Colour{#1}\large\phone}~}

%%%  \MakeMarkups[optionalComment]{prefixLetter}{textModifier}
%%%  One for each person: for example C for prefixLetter and \Colour{blue} for textModifier would be
%%%
%%%     \MakeMarkups[optionalComment]{C}{\Colour{blue}}
%%%
%%%  A possible use for optionalComment is to give the person's name.
%%%
%%%  "Disabling" a markup (or all of them) makes the document look as if that (those) markups had
%%%  been carried out. Replacements/deletions are done; footnotes, endnotes and t-comments are
%%%  removed; the document becomes black.
%%%
%%%  Disable all markups with macro \Bleck; also Green Room, Sargasso and Endnotes are suppressed.
%%%  Disable individual markup (rather than all via \Bleck) by eg \MakeMarkups[0]{C}{...}
%%%  Re-enable individual markups in spite of \Bleck with \MakeMarkups[1]{C}{...}
%%%
%%%  A help "how-to" can be printed any time after calling \MakeMarkups by \MarkupsHowto.
%%%  The "how-to" can be made shorter (just list the markups, no help) by \MarkupsHowtoPrintedtrue.
%%%

% Very sneaky!
\def\MarkupsHowto{} % How-to content, we add in every \MakeMarkups, use \MarkupHowto to print.
\newcommand{\MarkupsHowtoAdd}[1]{\expandafter\def\expandafter\MarkupsHowto\expandafter{\MarkupsHowto{}#1}} % adds to \MarkupsHowto

\newif\ifMarkupsHowtoPrinted %1121: Print help text only once. (Note: this is actually set to true when the how-to is _printed_.)
\newcommand\MakeMarkupsCalledtrue {\MarkupsHowtoPrintedtrue} % Temporary.
\newif\ifSuppress % Used to decide whether to suppress individual markups.

%%% Call this once for every markup'er you want to have.
\newcommand\MakeMarkups[3][.]{%1119

    % Suppress these markups if (Bleck OR [0]) and not [1].
     \Suppressfalse
     \ifBleck\Suppresstrue\fi
     \ifx0#1\Suppresstrue\fi
     \ifx1#1\Suppressfalse\fi
     
    % \Xx: Change to colour.
     \expandafter\providecommand\csname#2x\endcsname {} % 1613: Using providecommand this way allows MakeMarkups to be called more than once for a particular person.
     \ifSuppress\expandafter\renewcommand\csname#2x\endcsname{\relax}\else
                       \expandafter\renewcommand\csname#2x\endcsname{#3}\fi
                       
    % \X{#1}: Put #1 in colour.
     \expandafter\providecommand\csname#2\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2\endcsname[1]{##1}\else
                       \expandafter\renewcommand\csname#2\endcsname[1]{{\csname#2x\endcsname##1}}\fi

    % \Xd{#1}: Delete (strikeout) #1; needs ulem package.
     \expandafter\providecommand\csname#2d\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2d\endcsname[1]{\relax}\else
                       \expandafter\renewcommand\csname#2d\endcsname[1]{{\csname#2x\endcsname\sout{##1}}}\fi
                       
   % \Xr{#1}{#2}: Replace #1 with #2.
     \expandafter\providecommand\csname#2r\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2r\endcsname[2]{{##2}}\else
                       \expandafter\renewcommand\csname#2r\endcsname[2]{\csname#2d\endcsname{##1} \csname#2\endcsname{##2}}\fi

   % \Xi{#1}: Insert #1.
     \expandafter\providecommand\csname#2i\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2i\endcsname[1]{\relax}\else
                       \expandafter\renewcommand\csname#2i\endcsname[1]{\csname#2\endcsname{##1}}\fi

    % \Xt{#1}: Like \Xd{#1} but without strikeout; use where \Xf{#1} not allowed because e.g. "not in outer par mode".
     \expandafter\providecommand\csname#2t\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2t\endcsname[1]{\relax}\else
                       \expandafter\renewcommand\csname#2t\endcsname[1]{{\csname#2x\endcsname{\mbox{$\langle\!\langle$}##1{\csname#2x\endcsname\mbox{$\rangle\!\rangle$}}}}}\fi 

    % \Xb[#1]: Put bookmark in the margin, with optional parameter.
     \expandafter\providecommand\csname#2b\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2b\endcsname[1][empty]{\relax}\else 
                       \expandafter\renewcommand\csname#2b\endcsname[1][\empty]{\ifx\empty##1\empty
                       	\label{#2-bookmark} % With hyperlinks you can jump directly to your bookmark by clicking on an appropriate \pageref.
                              \marginpar [\raggedleft\csname#2\endcsname{{\footnotesize\fbox{#2 working here}}~$\Longrightarrow$}]
                                                {\csname#2\endcsname{$\Longleftarrow$~{\footnotesize\fbox{#2 working here}}}}
                       \else % No label if there's an explicit parameter.
                       	  % In general \ifx\empty#1\empty succeeds if the argument #1 is empty, or begins with \empty:
    			  % in the first case \if gets true for \empty=\empty;
    			  % in the second case it gets true for \empty=\empty (in #1), and possibly sticks in the rest of #1.
    			  % Anything else gives false.
                       	\marginpar [\raggedleft\csname#2\endcsname{\ifx\empty##1\empty\else\fbox{\tiny\parbox{8em}{\raggedright##1}}~\fi$\Longrightarrow$}]
                                                {\csname#2\endcsname{$\Longleftarrow$\ifx\empty##1\empty\else~{\tiny\fbox{\parbox{8em}{\raggedright##1}}}\fi}}\fi}\fi

    % \XTD: This person to do.
     \expandafter\providecommand\csname#2TD\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2TD\endcsname{\relax}\else
                       \expandafter\renewcommand\csname#2TD\endcsname{\csname#2\endcsname{\fbox{#2 to do}}}\fi

    % \XBar: Left by other people: delete when you're happy.
     \expandafter\providecommand\csname#2Bar\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2Bar\endcsname{\relax}\else
                       \expandafter\renewcommand\csname#2Bar\endcsname{\csname#2\endcsname{\scriptsize\XSolidBrush}}\fi

    % \Xf{#1}: Make coloured "footnote #1 to self".
     \expandafter\providecommand\csname#2f\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2f\endcsname[2][]{\relax}\else
      \expandafter\renewcommand\csname#2f\endcsname[2][\empty]{ % Have forgotten what the optional parameter was for.
        {\mbox{\csname#2x\endcsname\tiny$\boxtimes$}\marginpar{\hsize1cm\csname#2x\endcsname\fbox{\FnSym\footnotemark}}\relax 
        \footnotetext{\csname#2x\endcsname##2}}}\fi

    % \Xe{#1}: An endnote: like \Xf, but longer text #1 put at the end of the document.
     \expandafter\providecommand\csname#2e\endcsname {}% 1613.
     \ifSuppress\expandafter\renewcommand\csname#2e\endcsname[1]{\relax}\else%
      \expandafter\renewcommand\csname#2e\endcsname[1]{%
       \global\EndNotestrue%0831
       \mbox{\scriptsize\csname#2x\endcsname$\boxtimes$}\relax%
       \marginpar{\hsize1cm\csname#2x\endcsname\fbox{\EnSym\endnotemark%
                          \hypertarget{ENmark\thepage-\theendnote}{}~\hyperlink{ENtext\thepage-\theendnote}{{\Colour{blue}$\downarrow$}}}%
       }%
       {% 1641 Make \z,\zz local.
        \def\zz{\noexpand#3}%
%     \edef\z{~{\zz[Endnote \theendnote\ % Can't get this to work when #3 is several tokens. CCM 180521.
        \edef\z{~{[Endnote \theendnote\ %
        on p.\noexpand\hypertarget{ENtext\thepage-\theendnote}{}\thepage%
                    ~\noexpand\hyperlink{ENmark\thepage-\theendnote}{{\noexpand\Colour{blue}$\uparrow$}}]}%
        }%
        \expandafter\endnotetext\expandafter{\z\vspace{2ex}\\ ##1\newpage}%
       }%1641
      }\fi

    % \Xn{#1}: An endnote with no reference: like \Xe, but only a tiny marginal number is put in the text.
    % Useful in the final stages when you're removing notes (because they are distracting)
    % but still you might want to have a final look at the endnotes that were there
    % before you go for submission.
     \expandafter\providecommand\csname#2n\endcsname {}% 1613.
     \ifSuppress\expandafter\renewcommand\csname#2n\endcsname[1]{\relax}\else%
      \expandafter\renewcommand\csname#2n\endcsname[1]{%
       \global\EndNotestrue%0831
    %  \mbox{\scriptsize\csname#2x\endcsname$\boxtimes$}\relax
    %  \marginpar{\csname#2x\endcsname\fbox{\EnSym\endnotemark
    %                     \hypertarget{ENmark\thepage-\theendnote}{}~\hyperlink{ENtext\thepage-\theendnote}{{\Colour{blue}$\downarrow$}}}
    % }
    \marginpar{{\tiny\endnotemark}\hypertarget{ENmark\thepage-\theendnote}{}~\hyperlink{ENtext\thepage-\theendnote}{}}
       {% 1641 Make \z,\zz local.
        \def\zz{\noexpand#3}%
        \edef\z{~{\zz[Endnote (deferred) % \theendnote\ 
        from p.\noexpand\hypertarget{ENtext\thepage-\theendnote}{}\thepage%
    %\noexpand\hyperlink{ENmark\thepage-\theendnote}{{\noexpand\Colour{blue}$\uparrow$}}
        ]}%
        }%
        \expandafter\endnotetext\expandafter{\z\vspace{2ex}\\ ##1\newpage}%
       }%1641
      }\fi

    % Like \Xf and \Xe together --- Use \Xfe[<file name for endnote>]{Short footnote about file's contents.}
     \expandafter\providecommand\csname#2fe\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2fe\endcsname[2][]{\relax}\else %1538
      \expandafter\renewcommand\csname#2fe\endcsname[2][]{ % 1540: \File is local.
       \def\File{##1}\relax
       \ifx\File\empty\csname#2f\endcsname{##2}\else % 1536: Without file, behave like \Xf.
        \global\EndNotestrue %0831
        \mbox{\scriptsize\csname#2x\endcsname$\boxtimes$}
        \marginpar{\csname#2x\endcsname\fbox{\FnSym\footnotemark}}\relax
        \footnotetext{~\csname#2x\endcsname##2\
                             --- See [\EnSym\endnotemark\hypertarget{ENmark\thepage-\theendnote}{}
                             \kern-.2em\hyperlink{ENtext\thepage-\theendnote}{{\Colour{blue}$\downarrow$}}].}\relax
       { % 1641 Make \z,\zz local.
         \def\zz{\noexpand#3}
         \edef\z{~{\zz[Endnote~\thefootnote~on~p.\noexpand\hypertarget{ENtext\thepage-\theendnote}{}\thepage
                     ~\noexpand\hyperlink{ENmark\thepage-\theendnote}
                     {{\noexpand\Colour{blue}\kern-0.1em$\uparrow$}]}}
                     {\noexpand\footnotesize\noexpand\newline\noexpand\hspace*{2em} (~from file {\noexpand\tt\File.tex}~)}
         }    
         \expandafter\endnotetext\expandafter{\z~\par\input{##1}\newpage}
        } %1641
       \fi % 1536
      } % 1540
     \fi % 1538

    % "How-to" material printed by the first call to \MakeMarkups; suppress by \MarkupsHowtoPrintedtrue just before that first call.
    % Bleck removes the _whole footnote_ even if Suppress == false
     \ifSuppress\relax\else\ifBleck\relax\else%0749
      \MarkupsHowtoAdd{\par\csname#2t\endcsname{%1009
       $\backslash$\texttt{#2}$\cdots$\ markups are in \textbf{this} colour\ifx#1..\else\ifx1#1.\else, e.g.\ for #1.\fi\fi
       \ifMarkupsHowtoPrinted\relax\else %1121
        \global\MarkupsHowtoPrintedtrue %1121
        \begin{quote}\begin{tabular}{l@{\hspace{2em}}p{.7\linewidth}}
         \multicolumn{2}{l}{\texttt{$\backslash$MakeMarkups\ifx#1.\relax\else[#1]\fi\{#2\}\{{\it$\langle$colour command\/$\rangle$}\}}
         				 --- Defines the macros below:}\\
             & see comments at \texttt{$\backslash$MakeMarkups} definition. \\[1ex]
         \texttt{$\backslash$#2\{$\langle$text$\rangle$\}} & Sets \texttt{$\langle$text$\rangle$} in \texttt{#2}'s colour. \\
         \texttt{$\backslash$#2x} & Changes to \texttt{#2}'s colour (until end of context). \\
         \texttt{$\backslash$#2d\{$\langle$text$\rangle$\}} & Sets \texttt{$\langle$text$\rangle$} in \texttt{#2}'s colour with a strikethrough (i.e.\ delete). \\
         \texttt{$\backslash$#2r\{$\langle$this$\rangle$\}\{$\langle$that$\rangle$\}} &
          Strikes through \texttt{$\langle$this$\rangle$} and inserts \texttt{$\langle$that$\rangle$} (i.e.\ replace). \\
         \texttt{$\backslash$#2f\{$\langle$text$\rangle$\}} & Meta-comment: puts \texttt{$\langle$text$\rangle$} in a \texttt{#2}-footnote with a {\tiny$\boxtimes$} in the main text. \\
         \texttt{$\backslash$#2t\{$\langle$text$\rangle$\}} & Use for meta when  \texttt{$\backslash$#2f} isn't allowed (``Not in outer-par mode.'') \\
         \texttt{$\backslash$#2b[$\langle$optional$\rangle$]} & Marginal pointer, with label for hyper-linking directly there. \\
         \texttt{$\backslash$#2e\{$\langle$text$\rangle$\}} & Puts \texttt{$\langle$text$\rangle$} in a \texttt{#2}-endnote with a (big) $\boxtimes$ in the main text. \\[.5ex]
         \texttt{$\backslash$#2n\{$\langle$text$\rangle$\}} & Like \texttt{$\backslash$#2e}
         except there's no reference from the main text. Good for ``decluttering''
         when you still want to have the footnote- or endnote texts as reminders. \\[.5ex]
         \texttt{$\backslash$#2fe[$\langle$this$\rangle$]\{$\langle$that$\rangle$\}} & Makes a \texttt{$\backslash$#2f\{$\langle$that$\rangle$\}} that refers to a \\
           & \texttt{$\backslash$#2e\{$\langle$contents of file this.tex$\rangle$\}}. \\ 
           & Without the optional argument, acts as \texttt{$\backslash$#2f\{$\langle$that$\rangle$\}}. \\[.5ex]
         \texttt{$\backslash$#2Bar} & Inserts ``burn after reading'' symbol \csname#2Bar\endcsname, meaning
          \begin{quote}\begin{itemize}\setlength\itemsep{0pt}
           \item If yours is the only \csname#2Bar\endcsname\ in this (presumably someone else's) footnote, and you are happy that the footnote has been addressed,
           go ahead and comment-out the whole footnote. (The \csname#2Bar\endcsname\ is their request for you to ``approve and remove''.)
           \item If you are not happy, delete only your \csname#2Bar\endcsname\ and follow-on in the footnote
            (in your colour, i.e.\ with \texttt{$\backslash$#2x}) saying why you are not happy.
           \item If you are happy, but there are others' burn-after-reading symbols as well as yours, just delete yours; the other people have not yet responded.
          \end{itemize}
          \end{quote}
          The idea is that when everyone's happy, the last person will comment-out the meta-text. \\[0.5ex]
         \texttt{$\backslash$#2TD} & Inserts {\csname#2TD\endcsname}\ . \\
        \end{tabular}\end{quote}
       \fi
      }}%1009
     \fi\fi%0749
}%1119

\newcommand\Divider {~\vfill~\bigskip\hrule~\\\hrule~\bigskip} % For separating contributions in GreenRoom etc. Put in contributor's colour.

\newif\ifNoGreenRoom\newcommand\NoGreenRoom{\NoGreenRoomtrue}
\newcommand\MakeGreenRoom {\ifBleck\relax\else\ifNoGreenRoom\relax\else
% \cleardoublepage % Not necessary if \include'd.
% CCM Added "label-branding" 180524.
\newcommand\NewGRLabel[1] {\OldGRLabel{GreenRoom-##1}} % All Green-Room labels "branded".
 \newcommand\NewGRRef[1] % All Green-Room references take branded version if possible.
 {\expandafter\ifx\csname r@GreenRoom-##1\endcsname\relax\OldGRRef{##1}\else\OldGRRef{GreenRoom-##1}\fi}
 % Now swap them over.
 \let\OldGRLabel\label \let\label\NewGRLabel
 \let\OldGRRef\ref \let\ref\NewGRRef
 \hrule
 ~\\\begin{center}\Huge \hypertarget{GreenRoom}{Green Room}
 \end{center}~\\
 \hrule
\fi\fi}

\newcommand\EndGreenRoom  {\ifBleck\relax\else\ifNoGreenRoom\relax\else
% Swap them back.
\let\label\OldGRLabel
\let\ref\OldGRRef
\fi\fi}

\newif\ifNoEndNotes\newcommand\NoEndNotes{\NoEndNotestrue}
\newcommand\MakeEndNotes {\ifBleck\relax\else\ifNoEndNotes\relax\else
% \cleardoublepage % Not necessary if \include'd.
 \hrule\vspace{20pt}\begin{center}\ifEndNotes\Huge Endnotes\else\textit{No endnote macros were called in this run.}\fi\end{center}\vspace{20pt}\hrule
 {\parindent 0pt \parskip 2ex \def\enotesize{\normalsize} \def\notesname{} % Supress EndNotes title.
 \ifEndNotes\theendnotes\fi} %0831
\fi\fi}

\newif\ifNoSargasso\newcommand\NoSargasso{\NoSargassotrue}
\newcommand\MakeSargasso {
 % Localise labels and references to Sargasso itself, if possible.
 % Stuff In Sargasso might be a copy of earlier material, and we don't want the earlier labels to be overwritten.
 \hypertarget{Sargasso}{}
 \newcommand\NewLabel[1] {\OldLabel{Sargasso-##1}} % All Sargasso labels "branded".
 \newcommand\NewRef[1] % All Sargasso references take branded version if possible.
 {\expandafter\ifx\csname r@Sargasso-##1\endcsname\relax\OldRef{##1}\else\OldRef{Sargasso-##1}\fi}
 % Now swap them over.
 \let\OldLabel\label \let\label\NewLabel
 \let\OldRef\ref \let\ref\NewRef
 %
\ifBleck\end{document}\else\ifNoSargasso
\relax% \begin{center}\huge \textit{Sargasso suppressed in this run}\end{center}
\else
% \cleardoublepage % Not necessary if \include'd.
  \hrule
  ~\\\begin{center}\Huge Sargasso
  \end{center}~\\
  \hrule
 \fi\fi
}

\newcommand\EndSargasso  {\ifBleck\relax\else\ifNoSargasso\relax\else
% Swap them back.
\let\label\OldLabel
\let\ref\OldRef
\fi\fi}



\newcommand\EndDocument {\ifBleck\end{document}\fi} % Cut off the Green Room and the Sargasso when Bleck.

% For citations to be filled-in later: better than \cite{later} because \cite{later} generates undefined-reference warnings that might mask real ones.
% \Cite is -not- disabled by \Bleck, since \Bleck is supposed to make a version that is "OK to submit", and missing references is not "not OK".
% If necessary however (eg in a panic :-) you can enable \Bleck and disable \Cite, the latter by uncommenting the command following.
\newcommand\Cite[2][\empty] {{\Colour{red}\ifx#1\empty[#2]\else[#2,~#1]\fi}}
\newcommand\OpCit {[op.cit.]}
%\renewcommand\Cite[1] {\relax}

%%% End of \Markups

